Active nematics with quenched disorder

We introduce a two-dimensional active nematic with quenched disorder. We write the coarse-grained hydrodynamic equations of motion for slow variables, viz. density, and orientation. Disorder strength is tuned from zero to large values. Results from the numerical solution of equations of motion as well as the calculation of two-point orientation correlation function using linear approximation show that the ordered steady-state follows a disorder-dependent crossover from quasi long-range order (QLRO) to short-range order (SRO). Such crossover is due to the pinning of +1/2 and -1/2 topological defects in the presence of finite disorder, which breaks the system in uncorrelated domains. Finite disorder slows the dynamics of +1/2 defect, and it leads to slower growth dynamics. The two-point correlation functions for the density and orientation fields show good dynamic scaling but no static scaling for the different disorder strengths. Our findings can motivate experimentalists to verify the results and find applications in living and artificial apolar systems in the presence of a quenched disorder.

==> Active Nematic arxive/references.tex <==
\bibitem{naturecommindrani} C. J. O. Reichhardt and C. Reichhardt, Nature Physics 13 (2017).
\bibitem{naturecommindrani} A. Morin, N. Desreumaux, J. B. Caussin, and D. Bar- tolo, Nature Physics 13, 63 (2017), arXiv:1610.04404.
\bibitem{shradhapre2018} R. Das, M. Kumar, and S. Mishra, Physical Review E 98, 2 (2018), arXiv:1802.08861.
\bibitem{jtoner2018prl} J. Toner, N. Guttenberg, and Y. Tu, Physical Review Letters 121, 248002 (2018), arXiv:1805.10324.
\bibitem{jtoner2018pre} J. Toner, N. Guttenberg, and Y. Tu, Physical Review E 98, 1 (2018), arXiv:1805.10326.
\bibitem{fparuniprl2013} O. Chepizhko, E. G. Altmann, and F. Peruani, Physical Review Letters 110, 1 (2013), arXiv:1305.5707.
\bibitem{AnanyoMaitra2019} A. Maitra, Physical Review E 101, 1 (2020), arXiv:1910.07334.
\bibitem{dombrowski2004} C. Dombrowski, L. Cisneros, S. Chatkaew, R. E. Gold- stein, and J. O. Kessler, Physical Review Letters 93, 2 (2004).
\bibitem{sanchez2012} T. Sanchez, D. T. Chen, S. J. Decamp, M. Heymann, and Z. Dogic, Nature 491, 431 (2012).
\bibitem{sumino2012} Y. Sumino, K. H. Nagai, Y. Shitaka, D. Tanaka, K. Yoshikawa, H. Chat ́e, and K. Oiwa, Nature 483, 448 (2012).
\bibitem{imryma1975} Y. Imry and S. K. Ma, Physical Review Letters 35, 1399 (1975).
\bibitem{Rotunno2005} M. Rotunno, M. Buscaglia, C. Chiccoli, F. Mantegazza, P. Pasini, T. Bellini, and C. Zannoni, Physical Review Letters 94, 1 (2005).
\bibitem{kudrolli2003} D. L. Blair, T. Neicu, and A. Kudrolli, Physical Review E - Statistical Physics, Plasmas, Fluids, and Related In- terdisciplinary Topics 67, 6 (2003), arXiv:0203236 [cond- mat].
\bibitem{tsimiring2007} A. Sokolov, I. S. Aranson, J. O. Kessler, and R. E. Goldstein, Physical Review Letters 98, 1 (2007).
\bibitem{melanocytes} R. Komkemer, D. Kling, D. Kaufmann, and H. Gruler, European Physical Journal E 1, 215 (2000).

\bibitem{bsubtilis} L. H. Cisneros, J. O. Kessler, S. Ganguly, and R. E. Goldstein, Physical Review E - Statistical, Nonlinear, and Soft Matter Physics 83, 1 (2011).
\bibitem{Duclos2017} G. Duclos, C. Erlenka ̈mper, J. F. Joanny, and P. Sil- berzan, Nature Physics 13, 58 (2017).
\bibitem{Kawaguchi2017} K. Kawaguchi, R. Kageyama, and M. Sano, Nature 545, 327 (2017).
\bibitem{Saw2017} T. B. Saw, A. Doostmohammadi, V. Nier, L. Kocgozlu, S. Thampi, Y. Toyama, P. Marcq, C. T. Lim, J. M. Yeomans, and B. Ladoux, Nature 544, 212 (2017).
\bibitem{BlanchMercader2018} C. Blanch-Mercader, V. Yashunsky, S. Garcia, G. Duc- los, L. Giomi, and P. Silberzan, Physical Review Letters 120, 208101 (2018), arXiv:1711.01568.
\bibitem{Doostmohammadi2016} A. Doostmohammadi, S. P. Thampi, and J. M. Yeomans, Physical Review Letters 117, 1 (2016), arXiv:1601.04489.
\bibitem{DellArciprete2018} D. Dell’Arciprete, M. L. Blow, A. T. Brown, F. D. Far- rell, J. S. Lintuvuori, A. F. McVey, D. Marenduzzo, and W. C. Poon, Nature Communications 9, 1 (2018).
\bibitem{Yaman2019} Y. I. Yaman, E. Demir, R. Vetter, and A. Kocabas, Nature Communications 10, 1 (2019), arXiv:1811.12076. 
\bibitem{Li2019} H. Li, X. qing Shi, M. Huang, X. Chen, M. Xiao, C. Liu, H. Chat ́e, and H. P. Zhang, Proceedings of the National Academy of Sciences of the United States of America
116, 777 (2019).
\bibitem{shradhanjop} E. Bertin, H. Chat ́e, F. Ginelli, S. Mishra, A. Peshkov,
and S. Ramaswamy, New Journal of Physics 15 (2013),
10.1088/1367-2630/15/8/085032, arXiv:1305.0772.
\bibitem{husechateprl2004} H. Chat ́e, F. Ginelli, and R. Montagne, Physical Review
Letters 96, 1 (2006), arXiv:0603080 [cond-mat].
\bibitem{sriramadititonerepl2000} S. Ramaswamy, R. A. Simha, and J. Toner, Europhysics
Letters 62, 196 (2003), arXiv:0208573 [cond-mat].
\bibitem{Doostmohammadi2018} A. Doostmohammadi, J. Ign ́es-Mullol, J. M. Yeo- mans, and F. Sagu ́es, Nature Communications 9 (2018),
10.1038/s41467-018-05666-8.

\bibitem{shradhaprl} S. Mishra and S. Ramaswamy, Physical Review Letters 97, 1 (2006), arXiv:0603051 [cond-mat].
\bibitem{bray1994} A. J. Bray, Advances In Physics 43, 357 (1994).
]\bibitem{pggennes1993} P. de Gennes and J. Prost, The Physics of Liquid Crys- tals, International Series of Monogr (Clarendon Press,
1993).
\bibitem{lgiomiprl2013} L. Giomi, M. J. Bowick, X. Ma, and M. C. Marchetti,
Phys. Rev. Lett. 110, 228101 (2013).
\bibitem{shima2011} X.-q. Shi and Y.-q. Ma, (2010), arXiv:1011.5408.
\bibitem{rakeshscrep} R. Das, M. Kumar, and S. Mishra, Scientific Reports 7,
1 (2017).
\bibitem{Shi2013} X. Q. Shi and Y. Q. Ma, Nature Communications 4, 1
(2013).
\bibitem{Shi2014} X. Q. Shi, H. Chat ́e, and Y. Q. Ma, New Journal of
Physics 16 (2014), 10.1088/1367-2630/16/3/035003.
\bibitem{defecttopology} A. J. Vromans and L. Giomi, Soft Matter 12, 6490
(2016), arXiv:1507.05588.
\bibitem{vnarayan} N. M. Vijay Narayan, Sriram Ramaswamy, Science 317,
105 (2007).
\bibitem{shradhaphystrans} S. Mishra, S. Puri, and S. Ramaswamy, Philosoph-
ical Transactions of the Royal Society A: Mathemat- ical, Physical and Engineering Sciences 372 (2014), 10.1098/rsta.2013.0364.
\bibitem{pargellis1992} A. N. Pargellis, P. Finn, J. W. Goodby, P. Panizza, B. Yurke, and P. E. Cladis, Phys. Rev. A 46, 7765 (1992).
\bibitem{yurke1993} B. Yurke, A. N. Pargellis, T. Kovacs, and D. A. Huse, Phys. Rev. E 47, 1525 (1993).
\bibitem{Mbarma2000} D. Das and M. Barma, Phys. Rev. Lett. 85, 1602 (2000).
\bibitem{lgiomiprl2011} L. Giomi, L. Mahadevan, B. Chakraborty, and M. F.
Hagan, Phys. Rev. Lett. 106, 218101 (2011).
\bibitem{lgiomiiop2012} L. Giomi, L. Mahadevan, B. Chakraborty, and M. F.
Hagan, Nonlinearity 25, 2245 (2012).
\bibitem{chaikinlubenskey} P. M. Chaikin and T. C. Lubensky, Cambridge Univer-
sity Press (1995).
\bibitem{pgdegennes} P. G. de Gennes and J. Prost, Clarendon Press (1993).
\bibitem{chaikinlubenskey} G. B. Arfken and H. J. Weber, Mathematical Methods for Physics (ELSEVIER Academic Press, 2012) pp. 675– 739.


==> references.tex <==
\bibitem{naturecommindrani} C. J. O. Reichhardt and C. Reichhardt, Nature Physics 13 (2017).
\bibitem{naturecommindrani} A. Morin, N. Desreumaux, J. B. Caussin, and D. Bar- tolo, Nature Physics 13, 63 (2017), arXiv:1610.04404.
\bibitem{shradhapre2018} R. Das, M. Kumar, and S. Mishra, Physical Review E 98, 2 (2018), arXiv:1802.08861.
\bibitem{jtoner2018prl} J. Toner, N. Guttenberg, and Y. Tu, Physical Review Letters 121, 248002 (2018), arXiv:1805.10324.
\bibitem{jtoner2018pre} J. Toner, N. Guttenberg, and Y. Tu, Physical Review E 98, 1 (2018), arXiv:1805.10326.
\bibitem{fparuniprl2013} O. Chepizhko, E. G. Altmann, and F. Peruani, Physical Review Letters 110, 1 (2013), arXiv:1305.5707.
\bibitem{AnanyoMaitra2019} A. Maitra, Physical Review E 101, 1 (2020), arXiv:1910.07334.
\bibitem{dombrowski2004} C. Dombrowski, L. Cisneros, S. Chatkaew, R. E. Gold- stein, and J. O. Kessler, Physical Review Letters 93, 2 (2004).
\bibitem{sanchez2012} T. Sanchez, D. T. Chen, S. J. Decamp, M. Heymann, and Z. Dogic, Nature 491, 431 (2012).
\bibitem{sumino2012} Y. Sumino, K. H. Nagai, Y. Shitaka, D. Tanaka, K. Yoshikawa, H. Chat ́e, and K. Oiwa, Nature 483, 448 (2012).
\bibitem{imryma1975} Y. Imry and S. K. Ma, Physical Review Letters 35, 1399 (1975).
\bibitem{Rotunno2005} M. Rotunno, M. Buscaglia, C. Chiccoli, F. Mantegazza, P. Pasini, T. Bellini, and C. Zannoni, Physical Review Letters 94, 1 (2005).
\bibitem{kudrolli2003} D. L. Blair, T. Neicu, and A. Kudrolli, Physical Review E - Statistical Physics, Plasmas, Fluids, and Related In- terdisciplinary Topics 67, 6 (2003), arXiv:0203236 [cond- mat].
\bibitem{tsimiring2007} A. Sokolov, I. S. Aranson, J. O. Kessler, and R. E. Goldstein, Physical Review Letters 98, 1 (2007).
\bibitem{melanocytes} R. Komkemer, D. Kling, D. Kaufmann, and H. Gruler, European Physical Journal E 1, 215 (2000).

\bibitem{bsubtilis} L. H. Cisneros, J. O. Kessler, S. Ganguly, and R. E. Goldstein, Physical Review E - Statistical, Nonlinear, and Soft Matter Physics 83, 1 (2011).
\bibitem{Duclos2017} G. Duclos, C. Erlenka ̈mper, J. F. Joanny, and P. Sil- berzan, Nature Physics 13, 58 (2017).
\bibitem{Kawaguchi2017} K. Kawaguchi, R. Kageyama, and M. Sano, Nature 545, 327 (2017).
\bibitem{Saw2017} T. B. Saw, A. Doostmohammadi, V. Nier, L. Kocgozlu, S. Thampi, Y. Toyama, P. Marcq, C. T. Lim, J. M. Yeomans, and B. Ladoux, Nature 544, 212 (2017).
\bibitem{BlanchMercader2018} C. Blanch-Mercader, V. Yashunsky, S. Garcia, G. Duc- los, L. Giomi, and P. Silberzan, Physical Review Letters 120, 208101 (2018), arXiv:1711.01568.
\bibitem{Doostmohammadi2016} A. Doostmohammadi, S. P. Thampi, and J. M. Yeomans, Physical Review Letters 117, 1 (2016), arXiv:1601.04489.
\bibitem{DellArciprete2018} D. Dell’Arciprete, M. L. Blow, A. T. Brown, F. D. Far- rell, J. S. Lintuvuori, A. F. McVey, D. Marenduzzo, and W. C. Poon, Nature Communications 9, 1 (2018).
\bibitem{Yaman2019} Y. I. Yaman, E. Demir, R. Vetter, and A. Kocabas, Nature Communications 10, 1 (2019), arXiv:1811.12076. 
\bibitem{Li2019} H. Li, X. qing Shi, M. Huang, X. Chen, M. Xiao, C. Liu, H. Chat ́e, and H. P. Zhang, Proceedings of the National Academy of Sciences of the United States of America
116, 777 (2019).
\bibitem{shradhanjop} E. Bertin, H. Chat ́e, F. Ginelli, S. Mishra, A. Peshkov,
and S. Ramaswamy, New Journal of Physics 15 (2013),
10.1088/1367-2630/15/8/085032, arXiv:1305.0772.
\bibitem{husechateprl2004} H. Chat ́e, F. Ginelli, and R. Montagne, Physical Review
Letters 96, 1 (2006), arXiv:0603080 [cond-mat].
\bibitem{sriramadititonerepl2000} S. Ramaswamy, R. A. Simha, and J. Toner, Europhysics
Letters 62, 196 (2003), arXiv:0208573 [cond-mat].
\bibitem{Doostmohammadi2018} A. Doostmohammadi, J. Ign ́es-Mullol, J. M. Yeo- mans, and F. Sagu ́es, Nature Communications 9 (2018),
10.1038/s41467-018-05666-8.

\bibitem{shradhaprl} S. Mishra and S. Ramaswamy, Physical Review Letters 97, 1 (2006), arXiv:0603051 [cond-mat].
\bibitem{bray1994} A. J. Bray, Advances In Physics 43, 357 (1994).
]\bibitem{pggennes1993} P. de Gennes and J. Prost, The Physics of Liquid Crys- tals, International Series of Monogr (Clarendon Press,
1993).
\bibitem{lgiomiprl2013} L. Giomi, M. J. Bowick, X. Ma, and M. C. Marchetti,
Phys. Rev. Lett. 110, 228101 (2013).
\bibitem{shima2011} X.-q. Shi and Y.-q. Ma, (2010), arXiv:1011.5408.
\bibitem{rakeshscrep} R. Das, M. Kumar, and S. Mishra, Scientific Reports 7,
1 (2017).
\bibitem{Shi2013} X. Q. Shi and Y. Q. Ma, Nature Communications 4, 1
(2013).
\bibitem{Shi2014} X. Q. Shi, H. Chat ́e, and Y. Q. Ma, New Journal of
Physics 16 (2014), 10.1088/1367-2630/16/3/035003.
\bibitem{defecttopology} A. J. Vromans and L. Giomi, Soft Matter 12, 6490
(2016), arXiv:1507.05588.
\bibitem{vnarayan} N. M. Vijay Narayan, Sriram Ramaswamy, Science 317,
105 (2007).
\bibitem{shradhaphystrans} S. Mishra, S. Puri, and S. Ramaswamy, Philosoph-
ical Transactions of the Royal Society A: Mathemat- ical, Physical and Engineering Sciences 372 (2014), 10.1098/rsta.2013.0364.
\bibitem{pargellis1992} A. N. Pargellis, P. Finn, J. W. Goodby, P. Panizza, B. Yurke, and P. E. Cladis, Phys. Rev. A 46, 7765 (1992).
\bibitem{yurke1993} B. Yurke, A. N. Pargellis, T. Kovacs, and D. A. Huse, Phys. Rev. E 47, 1525 (1993).
\bibitem{Mbarma2000} D. Das and M. Barma, Phys. Rev. Lett. 85, 1602 (2000).
\bibitem{lgiomiprl2011} L. Giomi, L. Mahadevan, B. Chakraborty, and M. F.
Hagan, Phys. Rev. Lett. 106, 218101 (2011).
\bibitem{lgiomiiop2012} L. Giomi, L. Mahadevan, B. Chakraborty, and M. F.
Hagan, Nonlinearity 25, 2245 (2012).
\bibitem{chaikinlubenskey} P. M. Chaikin and T. C. Lubensky, Cambridge Univer-
sity Press (1995).
\bibitem{pgdegennes} P. G. de Gennes and J. Prost, Clarendon Press (1993).
\bibitem{chaikinlubenskey} G. B. Arfken and H. J. Weber, Mathematical Methods for Physics (ELSEVIER Academic Press, 2012) pp. 675– 739.

